Automatically Tailoring Static Analysis to Custom Usage Scenarios

In recent years, there has been significant progress in the development and industrial adoption of static analyzers. Such analyzers typically provide a large, if not huge, number of configurable options controlling the precision and performance of the analysis. A major hurdle in integrating static analyzers in the software-development life cycle is tuning their options to custom usage scenarios, such as a particular code base or certain resource constraints. In this paper, we propose a technique that automatically tailors a static analyzer, specifically an abstract interpreter, to the code under analysis and any given resource constraints. We implement this technique in a framework called TAILOR, which we use to perform an extensive evaluation on real-world benchmarks. Our experiments show that the configurations generated by TAILOR are vastly better than the default analysis options, vary significantly depending on the code under analysis, and most remain tailored to several subsequent code versions.

==> experiments_backup.tex <==
In this section, we present an extensive experimental evaluation
structured around the following research questions:
%
\begin{description}
\item[RQ1:] How do different optimization algorithms compare?
\item[RQ2:] How do optimized recipes compare with a default expert recipe?
\item[RQ3:] What are the characteristics of the optimized recipes?
\item[RQ4:] How does the timeout affect the optimization algorithms?
\item[RQ5:] How does the number of iterations affect the optimization
  algorithms?
\item[RQ6:] How do different settings affect the precision and
  performance of the abstract interpreter?
\item[RQ7:] Does an optimized recipe generalize to different versions
  of the same program?
\end{description}


%% ----------------------------------------------------------------
\subsection{Implementation}
\label{subsec:crab}
%% ----------------------------------------------------------------

%\todo{Maybe mention in the implementation section that Crab contains both local settings
%  per domain and global settings that apply to all domains.}

We implemented \tool by extending \crab~\cite{GurfinkelKahsai2015}, a parametric
framework for modular construction of abstract
interpreters\footnote{\crab is available at
  \url{https://github.com/seahorn/crab}.}.
%
We extended \crab with the ability to pass verification results
between recipe ingredients as well as with the four optimization
algorithms discussed in \secref{sec:Algorithms}. (We will make \tool
open source.)

Tab.~\ref{tab:allowed-parameter-values} shows all the settings and
values considered in our evaluation. For the initial recipe, \tool
uses Intervals and the \crab default values for all other settings (in
bold in the table). To make the search more efficient, we selected a
subset of all possible setting values for our experiments. However, to
ensure a representative subset, we consulted with the designer of
\crab.

\crab uses a DSA-based~\cite{GurfinkelNavas2017} pointer analysis and is able to
reason about array contents using array smashing.
%
\crab offers a wide range of logico-numerical domains, which are shown
in Fig.~\ref{fig:lattice}. The \texttt{bool} domain is the flat
Boolean domain, \texttt{ric} is a reduced product of Intervals and
Congruence~\cite{Granger1989}, and \texttt{term(int)} and
(\texttt{term(disInt)}) are instantiations of the Term~\cite{GangeNavas2016-Domain}
domain with \texttt{intervals} and \texttt{disInt}, respectively.
%
The default fixpoint engine of \crab implements the classical widening
Kleene iteration with narrowing.
%
Even though \crab provides a bottom-up inter-procedural analysis, our
evaluation uses the default intra-procedural analysis.

%% ----------------- possible parameter values

\begin{table}[t]
\centering
\scalebox{0.9}{
\begin{tabular}{l|l}
\textbf{Setting} & \textbf{Possible Values}\\
\hline
\textsc{\delays}    & $\lbrace \textbf{1}, 2, 4, 8, 16 \rbrace$ \\
\textsc{\narrowings} & $\lbrace 1, \textbf{2}, 3, 4 \rbrace$ \\
\textsc{\thresholds}  & $\lbrace \textbf{0}, 10, 20, 30, 40 \rbrace$ \\
\textsc{Backward Analysis}     & $\lbrace \textbf{OFF}, ON \rbrace$ \\
\textsc{Array Smashing} & $\lbrace OFF, \textbf{ON} \rbrace$ \\
\textsc{Abstract Domains}   & all domains in Fig.~\ref{fig:lattice} \\
\end{tabular}
}
\vspace{0.5em}
\caption{\crab settings and their possible values as used in our
  experiments. Default settings are shown in bold.}
\vspace{-2em}
\label{tab:allowed-parameter-values}
\end{table}

\begin{figure}[b]
\vspace{0.4em}
\scalebox{0.9}{
\begin{tikzpicture}[scale=.7]
  %% \node (one) at (0,2) {$1$};
  %% \node (a) at (-3,0) {$a$};
  %% \node (b) at (-1,0) {$b$};
  %% \node (c) at (1,0) {$c$};
  %% \node (d) at (3,0) {$d$};
  %% \node (zero) at (0,-2) {$0$};
  %% \draw (zero) -- (a) -- (one) -- (b) -- (zero) -- (c) -- (one) -- (d) -- (zero);

  \node (boxes) at (3,4) {\texttt{boxes}};
  \node (term-dis-int) at (5,3) {\texttt{term(disInt)}};
  \node (dis-int) at (3,2) {\texttt{disInt}};
  \node (poly) at (-3,4) {\texttt{polyhedra}};
  \node (oct) at (-3,3) {\texttt{octagons}};
  \node (zones) at (-3,2) {\texttt{zones}};
  \node (term-int) at (-1,2) {\texttt{term(int)}};
  \node (ric) at (1,2) {\texttt{ric}};
  \node (intervals) at (-1,0) {\texttt{intervals}};
  \node (bool) at (2,0) {\texttt{bool}};

  \draw (intervals) -- (ric) -- (intervals) -- (term-int) -- (intervals) -- (zones) -- (intervals) -- (dis-int) (zones) -- (oct) -- (poly) (dis-int) -- (term-dis-int) (dis-int) -- (boxes);

\end{tikzpicture}}

\caption{Comparing logico-numerical domains in \crab. A
  domain $d_1$ is less precise than $d_2$ if there is a path from
  $d_1$ to $d_2$ going upward, otherwise $d_1$ and $d_2$ are
  incomparable.}
\label{fig:lattice}
\end{figure}


%% ----------------------------------------------------------------
\subsection{Benchmark Selection}
\label{subsec:Benchmarks}
%% ----------------------------------------------------------------

To address our research questions, we systematically selected
popular C projects on GitHub. In particular, we chose the six most
starred C repositories with over 300 commits that we could
successfully build with the Clang-5.0 compiler. We give a short
description of each project in \tabref{tab:projects}.

For analyzing these projects using abstract interpretation, we needed
to introduce properties to be verified. For our purposes, we
instrumented these projects with four types of assertions that check
for common bugs; namely, division by zero, integer overflow, buffer
overflow, and use after free. Introducing assertions to check for
runtime errors such as these is common practice in program analysis
and verification.
%
(We will make our instrumentation tool
as well as all instrumented code available.)

As each project consisted of many files, we ran our experiments on a
random sample of 20 LLVM-bitcode files from each project, for a total
of 120 files. To ensure that each file was neither too trivial nor too
difficult for the underlying abstract interpreter, we only sampled
files with at least 20 assertions and at most 100. Additionally, to
guarantee all four assertion types (listed above) were included, we
required that the sum of assertions for each assertion type was at
least 70 across all files.

Overall, our benchmark suite of 120 files totals 1346 functions, 5557
assertions (on average 4 assertions per function), and 667,927 LLVM
instructions.
% \textcolor{red}{We do not know exactly how many lines of C code this
%   represents, as not every LLVM-bitcode file corresponds to a single C file.
%   However, the average C file from the projects we chose is 490 LOC, which
%   indicates our benchmarks are roughly 60,000 lines of C code.}
A more detailed description is given in
\tabref{tab:benchmarks}.
%

\begin{table}[t]
\centering
\scalebox{0.9}{
\begin{tabular}{l|l}
\textbf{Project} & \textbf{Description}\\
\hline
\textsc{curl}    & Tool for transferring data by URL\\
\textsc{darknet} & Convolutional neural-network framework\\
\textsc{ffmpeg}  & Multimedia processing tool\\
\textsc{git}     & Distributed version-control tool\\
\textsc{php-src} & PHP interpreter\\
\textsc{redis}   & Persistent in-memory database\\
\end{tabular}
}
\vspace{0.5em}
\caption{Overview of projects.}
\vspace{-1.5em}
\label{tab:projects}
\end{table}

\begin{table}[b]
\vspace{0em}
\centering
\scalebox{0.9}{
\begin{tabular}{l|S[table-format=2.0]|S[table-format=3.0]|S[table-format=3.0]}
\textbf{Project} & \textbf{Functions} & \textbf{Assertions}& \textbf{LLVM Instructions}\\
\hline
\textsc{curl}    & 306 & 787 & 50{,}541 \\
\textsc{darknet} & 130 & 958 & 55{,}847 \\
\textsc{ffmpeg}  & 103 & 888 & 27{,}653 \\
\textsc{git}     & 218 & 768 & 102{,}304 \\
\textsc{php-src} & 268 & 1031 & 305{,}943 \\
\textsc{redis}   & 321 & 1125 & 125{,}639 \\
\hline
\textbf{Total}   & 1346 & 5557 & 667{,}927
\end{tabular}
}
\vspace{0.5em}
\caption{Benchmark characteristics (20 files per project). The last
  three columns show the number of functions, assertions, and LLVM
  instructions in the analyzed files.}
\vspace{-1.0em}
\label{tab:benchmarks}
\end{table}

% Finally, \crab offers both a bottom-up and top-down
% inter-procedural analysis as described in
% Sec.~\ref{sec:abstract-interpreters}. However, our evaluation only
% exercises the intra-procedural variant. We tried the bottom-up
% analysis but results were not different from using the
% intra-procedural analysis. The top-down analysis has been recently
% implemented in \crab and we plan to evaluate it in future work.

%% %% ----------------------------------------------------------------
%% \subsection{Setup}
%% \label{subsec:Setup}
%% %% ----------------------------------------------------------------

%% \jorge{We should have a subsection called ``Prototype or
%%   Implementation'' or something like that. There, we mention that we
%%   have a new tool called superCrab. It has to be clear that we have a
%%   new tool!}

%% We performed all experiments on a 32 core \mbox{Intel}
%%     \textregistered~Xeon \textregistered~E5-2667 v2 CPU~@~3.30GHz machine
%%   with 264~GB of memory, running Ubuntu 16.04.1 LTS.
%% ----------------------------------------------------------------
\subsection{Results}
\label{subsec:Results}
%% ----------------------------------------------------------------
We now present experimental results for each research question.
%
We performed all experiments on a 32-core \mbox{Intel}
\textregistered~Xeon \textregistered~E5-2667 v2 CPU~@~3.30GHz machine
with 264GB of memory, running Ubuntu 16.04.1 LTS.

\textbf{RQ1: Comparison of optimization algorithms.}
%
We compare the four optimization algorithms that we described in
\secref{sec:Algorithms}: random sampling (\textsc{rs}), domain-aware
random sampling (\textsc{dars}), simulated annealing (\textsc{sa}),
and hill climbing (\textsc{hc}).

For this experiment, we ran \tool with each optimization algorithm on
our 120 benchmark files. We enabled optimization at the granularity of
files and enforced a timeout of 5 minutes per recipe. In
\algoref{alg:optimize-algorithm}, we set \textit{maxRcpLen} to 3,
\textit{domainSteps} to 5, and \textit{settingIters} to 10. Each
  algorithm was seeded with the same random seed.

The results are shown in \figsref{fig:alg-comparison},
\ref{fig:alg-best-iterations}, \ref{fig:alg-best-time}, and
\ref{fig:alg-total-time}. Consider only the bars for the 5-minute
timeout (in green).  \figref{fig:alg-comparison} shows the number of
assertions that were verified with the best recipe found by each
algorithm (\textsc{dars}, \textsc{rs}, \textsc{sa}, and
\textsc{hc}). (\textsc{exp} should be ignored for now.) The
random-sampling algorithms are shown to find better recipes than the
others, with \textsc{dars} being the most effective. Hill climbing is
less effective since it gets stuck in local cost minima despite
restarts. Simulated annealing is the least effective because it slowly
climbs up the poset toward more precise domains (see
\algoref{alg:recipe-generation-algorithm}). Note that, even with
\textsc{dars}, we are able to verify 953 assertions out of a total of
5557 ($\sim$17\%). This relatively low percentage is due to the
intra-procedural nature of our analysis. Specifically, every function
is analyzed for all possible calling contexts. As a result, an
unverified assertion might not hold for calling contexts that do not
occur in the program. Even if it does hold, it might be too
challenging to verify for any calling context.

\figsref{fig:alg-best-iterations} and \ref{fig:alg-best-time} show the
average number of iterations and the average time it takes each
optimization algorithm to generate the best recipe. In
\figref{fig:alg-total-time}, we show the total time that each
algorithm takes for all iterations. \textsc{dars} takes longer than
all other algorithms. This is due to generating more precise recipes,
which typically take longer to run. This is also why it verifies the
most assertions (\figref{fig:alg-comparison}).

%% We repeated this experiment while persisting invariants at each basic
%% block. Surprisingly, this did not affect \figref{fig:alg-comparison}
%% at all, in other words, simply converting verified assertions into
%% assumptions for the next recipe ingredient does not have a negative
%% impact on the verification results in these benchmarks.
%% %
%% However, we observed that persisting invariants does slightly impact
%% the total time shown in \figref{fig:alg-total-time}. In particular,
%% the different algorithms are either 3--4\% slower or faster. Both
%% outcomes make sense. An algorithm runs slower when persisting
%% invariants if these do not prove useful to the subsequent recipe
%% ingredient. If they are useful, then the subsequent analysis leverages
%% them and runs faster.

%% --------- absolute winners

%% \begin{figure}[t]
%% \centering
%% \scalebox{0.85}{
%%   \begin{tikzpicture}
%%     \begin{axis}[
%%       % ybar stacked,
%%       ybar,
%%       xticklabels={\textsc{rs},\textsc{dars},\textsc{sa},\textsc{hc},\textsc{exp}},
%%       xtick=data,
%%       % xticklabel style={rotate=-45},
%%       ylabel={\textbf{Number of verified files}},
%%       legend cell align=left,
%%       axis y line*=none,
%%       axis x line*=bottom,
%%       width=10cm,
%%       height=7cm,
%%       ymin=0,
%%       ymax=30,
%%       ytick distance=15,
%%       bar width=0.6cm,
%%       area legend,
%%       nodes near coords,
%%       legend style={legend pos=north east,font=\small, draw=none, legend columns=-1}
%%       % every node near coord/.append style={rotate=90, anchor=west}
%%       ]

%%       \pgfplotstableread{data/absolute-winners.dat}\unsoundness

%%       \addplot+[ybar, Blue, pattern color=Blue, pattern=north east lines]
%%           table[x expr=\coordindex, y=x5] from \unsoundness;

%%       \addplot+[ybar, Green, pattern color=Green, pattern=north west lines]
%%           table[x expr=\coordindex, y=x4] from \unsoundness;

%% %      \addplot+[ybar, DarkOrange, pattern color=DarkOrange, pattern=crosshatch]
%% %          table[x expr=\coordindex, y=x3] from \unsoundness;

%%       \legend{1sec, 5min} %, 10min}
%%     \end{axis}
%%   \end{tikzpicture}
%% }
%% %\vspace{-1em}
%% \caption{Comparison of the number of files that are only verified with
%%   the best recipe generated by an optimization algorithm or with the
%%   expert recipe, for varying timeouts.}
%% \label{fig:alg-wins}
%% \vspace{-0.5em}
%% \end{figure}



%% \begin{figure}[t]
%% \centering
%% \DTLpiechart{variable=\quantity,outerlabel=\name,innerratio=0.7}{dataBO}{
%% \name=Name,\quantity=Quantity}
%% \caption{Most used domains (buffer overflow)}
%% \label{fig:most-used-domains-bo}
%% \end{figure}

%% \begin{figure}[t]
%% \centering
%% \DTLpiechart{variable=\quantity,outerlabel=\name,innerratio=0.7}{dataDBZ}{
%% \name=Name,\quantity=Quantity}
%% \caption{Most used domains (division by zero)}
%% \label{fig:most-used-domains-dbz}
%% \end{figure}

%% --------- Combined Opt Algo comparison graph for number of safe checks

\begin{figure}[t]
\centering
\scalebox{0.75}{
  \begin{tikzpicture}
    \begin{axis}[
      % ybar stacked,
      ybar,
      xticklabels={\textsc{dars},\textsc{rs},\textsc{hc},\textsc{sa},\textsc{exp}},
      xtick=data,
      % xticklabel style={rotate=-45},
      ylabel={\textbf{Number of verified assertions}},
      legend cell align=left,
      axis y line*=none,
      axis x line*=bottom,
      width=10cm,
      height=5.5cm,
      ymin=0,
      ymax=1400,
      ytick distance=200,
      bar width=0.6cm,
      area legend,
      nodes near coords,
      legend style={legend pos=north east,font=\small, draw=none, legend columns=-1}
      % every node near coord/.append style={rotate=90, anchor=west}
      ]

      \pgfplotstableread{data/ver-assert-compariosn.dat}\unsoundness

      \addplot+[ybar, Blue, pattern color=Blue, pattern=north east lines]
          table[x expr=\coordindex, y=x5] from \unsoundness;

      \addplot+[ybar, Green, pattern color=Green, pattern=north west lines]
          table[x expr=\coordindex, y=x4] from \unsoundness;

%      \addplot+[ybar, DarkOrange, pattern color=DarkOrange, pattern=crosshatch]
%          table[x expr=\coordindex, y=x3] from \unsoundness;

      \legend{1sec, 5min} %, 10min}
    \end{axis}
  \end{tikzpicture}
}
\vspace{-0.5em}
\caption{Comparison of the number of assertions verified with the best
  recipe generated by the different optimization algorithms and with
  an expert recipe, for varying timeouts.}
\label{fig:alg-comparison}
\vspace{-0.5em}
\end{figure}

%% --------- Average number of iterations required to reach the best config - Algo Comparison
\begin{figure}[t]
\centering
\scalebox{0.75}{
  \begin{tikzpicture}
    \begin{axis}[
      % ybar stacked,
      ybar,
      xticklabels={\textsc{dars},\textsc{rs},\textsc{hc},\textsc{sa}},
      xtick=data,
      % xticklabel style={rotate=-45},
      ylabel={\textbf{Average number of iterations}},
      legend cell align=left,
      axis y line*=none,
      axis x line*=bottom,
      width=10cm,
      height=5.5cm,
      ymin=0,
      ymax=30,
      ytick distance=15,
      bar width=0.6cm,
      area legend,
      nodes near coords,
      legend style={legend pos=north east,font=\small, draw=none, legend columns=-1}
      % every node near coord/.append style={rotate=90, anchor=west}
      ]

      \pgfplotstableread{data/alg-avg-best-iter.dat}\unsoundness

      \addplot+[ybar, Blue, pattern color=Blue, pattern=north east lines]
          table[x expr=\coordindex, y=x5] from \unsoundness;

      \addplot+[ybar, Green, pattern color=Green, pattern=north west lines]
          table[x expr=\coordindex, y=x4] from \unsoundness;

%      \addplot+[ybar, DarkOrange, pattern color=DarkOrange, pattern=crosshatch]
%          table[x expr=\coordindex, y=x3] from \unsoundness;

      \legend{1sec, 5min} % , 10min}
    \end{axis}
  \end{tikzpicture}
}
\vspace{-0.5em}
\caption{Comparison of the average number of iterations that each
  algorithm needs to find the best recipe, for varying timeouts.}
\label{fig:alg-best-iterations}
\vspace{-1.5em}
\end{figure}

\textbf{RQ2: Comparison of optimized recipes with a default expert recipe.}
%
We compare the best recipe found by each optimization algorithm with
an expert recipe, i.e., the default settings in \crab as defined by
its designer. The expert recipe uses a combination of two domains,
namely, the reduced product of the Boolean and Zones domains. The
other default settings are shown in
Tab.~\ref{tab:allowed-parameter-values}.

In \figref{fig:alg-comparison}, \textsc{exp} represents this expert
recipe. All optimization algorithms are significantly more effective
than \textsc{exp}, which is proof of the fact that a single recipe
cannot be suitable for all code. Since it proves fewer assertions, the
\textsc{exp} recipe is on average faster than the optimized recipes.
%
\figref{fig:compare-assertions} shows the comparison of the total
number of assertions that were verified by an optimized versus the
expert recipe with a 5-minute timeout. For example, the \textsc{dars}
and \textsc{exp} recipes were both able to verify 378 assertions, but
575 assertions were verified only by \textsc{dars} and 79 only by
\textsc{exp}.

%% --------- Average time required to run all the iterations - Algo Comparison
\begin{figure}[t]
\centering
\scalebox{0.75}{
  \begin{tikzpicture}
    \begin{axis}[
      % ybar stacked,
      ybar,
      xticklabels={\textsc{dars},\textsc{rs},\textsc{hc},\textsc{sa}},
      xtick=data,
      % xticklabel style={rotate=-45},
      ylabel={\textbf{Average time (seconds)}},
      legend cell align=left,
      axis y line*=none,
      axis x line*=bottom,
      width=10cm,
      height=5.5cm,
      ymin=0,
      ymax=800,
      ytick distance=200,
      bar width=0.6cm,
      area legend,
      nodes near coords,
      legend style={legend pos=north east,font=\small, draw=none, legend columns=-1}
      % every node near coord/.append style={rotate=90, anchor=west}
      ]

      \pgfplotstableread{data/alg-best-time.dat}\unsoundness

      \addplot+[ybar, Blue, pattern color=Blue, pattern=north east lines]
          table[x expr=\coordindex, y=x5] from \unsoundness;

      \addplot+[ybar, Green, pattern color=Green, pattern=north west lines]
          table[x expr=\coordindex, y=x4] from \unsoundness;

%      \addplot+[ybar, DarkOrange, pattern color=DarkOrange, pattern=crosshatch]
%          table[x expr=\coordindex, y=x3] from \unsoundness;

      \legend{1sec, 5min }  %, 10min}
    \end{axis}
  \end{tikzpicture}
}
\vspace{-0.5em}
\caption{Comparison of the average time (in seconds) that each
  algorithm requires to find the best recipe, for varying timeouts.}
\label{fig:alg-best-time}
\vspace{-0.5em}
\end{figure}

%% --------- Average time required to run all the iterations - Algo Comparison
\begin{figure}[t]
\centering
\scalebox{0.75}{
  \begin{tikzpicture}
    \begin{axis}[
      % ybar stacked,
      ybar,
      xticklabels={\textsc{dars},\textsc{rs},\textsc{hc},\textsc{sa}},
      xtick=data,
      % xticklabel style={rotate=-45},
      ylabel={\textbf{Total time (seconds)}},
      legend cell align=left,
      axis y line*=none,
      axis x line*=bottom,
      width=10cm,
      height=5.5cm,
      ymin=0,
      ymax=1400,
      ytick distance=200,
      bar width=0.6cm,
      area legend,
      nodes near coords,
      legend style={legend pos=north east,font=\small, draw=none, legend columns=-1}
      % every node near coord/.append style={rotate=90, anchor=west}
      ]

      \pgfplotstableread{data/alg-total-time.dat}\unsoundness

      \addplot+[ybar, Blue, pattern color=Blue, pattern=north east lines]
          table[x expr=\coordindex, y=x5] from \unsoundness;

      \addplot+[ybar, Green, pattern color=Green, pattern=north west lines]
          table[x expr=\coordindex, y=x4] from \unsoundness;

%      \addplot+[ybar, DarkOrange, pattern color=DarkOrange, pattern=crosshatch]
%          table[x expr=\coordindex, y=x3] from \unsoundness;

      \legend{1sec, 5min} %, 10min}
    \end{axis}
  \end{tikzpicture}
}
\vspace{-0.5em}
\caption{Comparison of the total time (in seconds) that each algorithm
  requires for all iterations, for varying timeouts.}
\vspace{-1.5em}
\label{fig:alg-total-time}
\end{figure}

To better evaluate the optimality of our recipes, we also compared
with the most precise \crab configuration. It uses the most precise
domains from \figref{fig:lattice} (i.e., \texttt{bool},
\texttt{polyhedra}, \texttt{term(int)}, \texttt{ric}, \texttt{boxes},
and \texttt{term(disInt)}) in a recipe of 6 ingredients and assigns
the most precise values to all other settings from
\tabref{tab:allowed-parameter-values}. We gave a 30-minute timeout to
this recipe. For 21 out of 120 files, the most precise recipe ran out
of memory (264GB). For 86 files, it terminated in less than 5 minutes,
and for 13 files, it took longer to terminate (within 30 minutes). We
compared the number of assertions that are verified by our
\textsc{dars} recipes (which do not exceed 5 minutes) and by the most
precise recipe. For the 86 files, our recipes prove 618 assertions,
whereas the most precise recipe proves 534 assertions. For the 13
files, our recipes prove 119 assertions, whereas the most precise
recipe proves 98. Consequently, our (in theory) less precise and more
efficient recipes prove more assertions for those files where the most
precise recipe does not run out of memory. This is mainly because the
coefficients of polyhedra might overflow, in which case the
constraints are typically ignored by abstract interpreters. In such
cases, theoretically less precise domains might result in more precise
results. This might also occur when different domains use different
widening operations~\cite{MonniauxLeGuen2012,AmatoRubino2018}.


\textbf{RQ3: Characteristics of optimized recipes.}
%
To understand their characteristics, we manually inspected all
optimized recipes generated by \textsc{dars} since they verified the
most assertions.

\textsc{dars} generated recipes of length greater than 1 for 61 out of
120 files. Out of these, 37 are of length 2 and 24 of length 3.
%
To evaluate the impact of the recipe length, we also ran \textsc{dars}
with $\mathit{maxRcpLen}$ from \algoref{alg:optimize-algorithm} set to
1. This reduced the number of verified assertions to 884 (9.2\%).

Coming back to the experiment with a maximum recipe length of 3, 55\%
of the ingredients enable array smashing, and 32\% enable backward
analysis. For 77\% of all best recipes, \delays is not set to the
default value of 1.

\figref{fig:most-used-domains} shows how often (in percentage) each
abstract domain occurs in a best recipe found by \textsc{dars}. We can
observe that all ten domains are used, which highlights that there
does not exist a single recipe for analyzing all code. This is also
true even when instrumenting the benchmarks only with one assertion
type, e.g., those that check for integer overflow (see
\figref{fig:most-used-domains-IO}). In both pie charts,
\texttt{intervals} is used less since it is the least precise
non-boolean domain in the poset (\figref{fig:lattice}).

% -------------------- Expert Assertion Experiment

\begin{figure}[t]
\centering
\scalebox{0.75}{
\begin{tikzpicture}
\begin{axis}[
   xbar stacked,
	 ytick=data,
	 yticklabels={\textsc{dars}, \textsc{rs}, \textsc{hc}, \textsc{sa}},
     ylabel={\textbf{Optimization algorithms}},
     legend cell align=left,
     axis y line*=none,
     axis x line*=bottom,
     width=10cm,
     height=6cm,
     xmin=0,
     xmax=1100,
     ymax=5,
     xtick distance=500,
     bar width=0.6cm,
     area legend,
     legend style={legend pos=north east,font=\small, draw=none, legend columns=-1}
   ]

\addplot+[xbar, Green!70] plot coordinates {(575, 1) (578, 2) (535, 3) (526, 4)};

\addplot+[xbar, DarkOrange!70] plot coordinates {(378, 1) (366, 2) (379, 3) (386, 4)};

\addplot+[xbar, Red!70] plot coordinates {(79, 1) (91, 2) (78, 3) (71, 4)};

\legend{\tool, Both, \textsc{exp}}

\coordinate (A) at (300,1);
\coordinate (B) at (300,2);
\coordinate (C) at (300,3);
\coordinate (D) at (300,4);

\coordinate (AA) at (750,1);
\coordinate (BB) at (750,2);
\coordinate (CC) at (750,3);
\coordinate (DD) at (750,4);

\coordinate (AAA) at (995,1);
\coordinate (BBB) at (990,2);
\coordinate (CCC) at (955,3);
\coordinate (DDD) at (950,4);


\end{axis}

\node at (A) {575};
\node at (B) {578};
\node at (C) {535};
\node at (D) {526};

\node at (AA) {378};
\node at (BB) {366};
\node at (CC) {379};
\node at (DD) {386};

\node at (AAA) {79};
\node at (BBB) {91};
\node at (CCC) {78};
\node at (DDD) {71};

\end{tikzpicture}
}
\vspace{-0.5em}
\caption{Comparison of the number of assertions verified by an
  optimized vs. the expert recipe.}
\label{fig:compare-assertions}
\vspace{-1.0em}
\end{figure}

We also inspected which domain combinations are frequently used in the
best recipes. One common pattern is combinations between \texttt{bool}
and numerical domains (18 occurrences). This empirically validates
\crab's design of using a reduced-product combination with
\texttt{bool} when selecting any numerical domain. Similarly, we
observed 2 occurrences of \texttt{term(disInt)} together with
\texttt{zones}, which is another built-in combination in
\crab. Interestingly, the less powerful variants of combining
\texttt{disInt} with \texttt{zones} (3 occurrences) and
\texttt{term(int)} with \texttt{zones} (6 occurrences) seem to be
sufficient in many cases. Finally, we observed 8
occurrences of \texttt{polyhedra} or \texttt{octagons} with
\texttt{boxes}, which is not surprising as these are the most precise
convex and non-convex domains. Our approach is, thus, not only
useful for users, but also for designers of abstract interpreters by
inspiring new domain combinations.

% \todo{Jorge, please explain.}
% %
% We observed:
% \begin{itemize}
% \item boolean with another domain: 20 times
% \item zones + dis-int: 7 times
% \item dis-int + term(int): 6 times
% \item polyhedra + boxes: 3 times
% \item term(dis-int) + zones: 2 times
% \end{itemize}

% \jorge{(Informal) comments:} \crab organizes the logico-numerical
% domains by having a fixed reduced product between the flat Boolean
% domain and a numerical domain. The Boolean domain is fixed but the
% numerical domain is an user parameter. The reduction between the
% Boolean and the numerical domain is also fixed (it's independent from
% the particular numerical domain). Our optimization algorithms figure
% out that combining boolean with another domain is a good thing to
% do. Also interestingly, our optimization algorithms decides to combine
% term(dis-int) + zones. In fact, \crab offers a customized numerical
% domain that performs the reduced product of exactly these two
% domains. The reduction is optimized to avoid propagating redundant
% constraints between the two domains. For instance, term(X) (for any X
% domain) can infer equalities that zones cannot infer, and
% vice-versa\jorge{Maybe explain which equalities?}. Related to this,
% our optimization algorithms finds out that zones + dis-int is enough
% in several cases. The difference between term(dis-int) and dis-int is
% that the former infers equalities between expressions and the latter
% does not but both infer some simple disjunctions of intervals. (e.g.,
% $x < 10$ or $x > 20$) due to the use of dis-int. In 7 cases, our
% optimization algorithms finds out that inferring equalities between
% expressions does not pay off. Finally, polyhedra + boxes makes sense
% since they are the most precise convex and non-convex domains. It
% would make a lot sense to have a combination boxes + X where X is a
% domain that can infer relationships between variables (e.g., zones,
% octagons, polyhedra, etc)

%% \jorge{I cannot make a lot of sense of dis-int +
%%   term(int). term(dis-int) should have the same precision and similar
%%   efficiency. Maybe in those cases the cost was very similar to
%%   term(dis-int) but the algorithm chose dis-int + term(int) for a
%%   small difference.}

%% \jorge{it would be interesting if there is a recipe with bool +
%%   boxes. Boxes is the only numerical domain that reason natively about
%%   boolean variables. The only reason to have bool + boxes would be if
%%   bool can remove a lot paths so that boxes is then more efficient.}

\textbf{RQ4: Varying the timeout of the optimization algorithms.}
%
We experimented with varying the timeout per recipe. We used the same
setup as in RQ1 but changed the timeout to 1~second. The results are
shown in \figsref{fig:alg-comparison}, \ref{fig:alg-best-iterations},
\ref{fig:alg-best-time}, and \ref{fig:alg-total-time}.
%
As shown in \figref{fig:alg-comparison}, the algorithms are able to
find recipes that on average verify 66\% of the assertions that are
verified with a 5-minute timeout. This suggests that many
assertions are easy to prove with relatively imprecise recipes
that do not reach this short timeout. The other 44\% of the
assertions, however, require more expensive recipes.

The timeout also affects the length of the optimized recipes. In
particular, \textsc{dars} generates recipes of length greater than 1
for 32 out of 120 files. Out of these, 29 have a recipe of length 2,
and only 3 of length 3. Compared to the 5-minute timeout, this shows a 48\% reduction in the number of recipes of
length greater than 1.

Note that we select 1-second and 5-minute timeouts as representative
of different usage scenarios, i.e., modifying code in the editor and
building one of the benchmark projects. We also experimented with
larger timeouts, but the results were almost the same as for the
5-minute timeout since the vast majority of recipes do not exceed it.

\textbf{RQ5: Varying the number of iterations of the optimization algorithms.}
%
\figsref{fig:alg-iter-comparison} and
\ref{fig:alg-iter-best-iterations} compare the optimization algorithms
for varying numbers of iterations. For this experiment, we used the
same setup as in RQ1, except for the number of iterations.  We set
\textit{domainSteps} to 10 and \textit{settingIters} to 20.

\figref{fig:alg-iter-comparison} shows that with 80 iterations a relatively small number of
additional assertions are verified. In fact, we expect the
algorithms to eventually converge on the assertions that are provable given the constraints
(e.g., with respect to the time limit and the precision of the available
domains). \figref{fig:alg-iter-best-iterations} shows the number of iterations required
for each algorithm to find the best recipe, which indicates that a few assertions require
more specialized recipes to be proved.

\DTLloaddb{data}{data/most-used-domains.csv}
\DTLloaddb{dataBO}{data/most-used-domains-bufferoverflow.csv}
\DTLloaddb{dataDBZ}{data/most-used-domains-divbyzero.csv}
\DTLloaddb{dataIO}{data/most-used-domains-intoverflow.csv}

\begin{figure}[t]
\centering
\scalebox{0.75}{
\DTLpiechart{variable=\quantity,outerlabel=\name,innerratio=0.7,radius=1.65cm}{data}{
  \name=Name,\quantity=Quantity}}
\vspace{-0.5em}
\caption{Occurrence of domains (in percentage) in the best recipes
  found by \textsc{dars} for all assertion types.}
\vspace{-1em}
\label{fig:most-used-domains}
\end{figure}


\begin{figure}[t]
  \centering
  \scalebox{0.75}{
\DTLpiechart{variable=\quantity,outerlabel=\name,innerratio=0.7,radius=1.65cm}{dataIO}{
  \name=Name,\quantity=Quantity}}
\vspace{-0.5em}
\caption{Occurrence of domains (in percentage) in the best recipes
  found by \textsc{dars} for integer-overflow assertions.}
\vspace{-1em}
\label{fig:most-used-domains-IO}
\end{figure}

The optimized recipes that \textsc{dars} generates differ from those
it generates for 40 iterations (RQ3) in the following way. The recipes
of length greater than 1 are now 62 (instead of 61), with 35 of length
2 and 27 of length 3. Therefore, even though the algorithm performed
more iterations for each recipe length, it did not find better recipes
of shorter length.
%
Regarding domain combinations, we did not observe significant
differences with respect to those discussed in RQ3.

\textbf{RQ6: Quantifying the effect of different settings.}
%
To evaluate the impact of different settings, we took the best recipes
found by \textsc{dars} and mutated each recipe setting individually.
%
In particular, for each setting in
\tabref{tab:allowed-parameter-values}, we tried all possible values.
We also replaced each domain with all other comparable domains in the
poset of \figref{fig:lattice}.
%
For example, for a recipe including \texttt{zones}, we tried
\texttt{octagons}, \texttt{polyhedra}, and \texttt{intervals}.
%
In addition, we tried all possible orderings of the recipe
ingredients, which in theory could produce different results. We
observed whether these changes resulted in a difference in the
precision and performance of the analyzer.

\figref{fig:toggle-best-recipe} shows the results of this experiment,
broken down by setting. Equal (in orange) indicates that the mutated
recipe proves the same number of assertions within $\pm 5$ seconds of
the original. Positive (in green) indicates that it either proves more
assertions or the same number of assertions at least $5$ seconds
faster.  Negative (in red) indicates that the mutated recipe either
proves fewer assertions or the same number of assertions at least $5$
seconds slower.

%% --------- Combined Opt Algo comparison graph for number of safe checks

\begin{figure}[t]
\centering
\scalebox{0.75}{
  \begin{tikzpicture}
    \begin{axis}[
      % ybar stacked,
      ybar,
      xticklabels={\textsc{dars},\textsc{rs},\textsc{hc},\textsc{sa}},
      xtick=data,
      ylabel={\textbf{Number of verified assertions}},
      legend cell align=left,
      axis y line*=none,
      axis x line*=bottom,
      width=10cm,
      height=5.5cm,
      ymin=0,
      ymax=1400,
      ytick distance=700,
      bar width=0.6cm,
      area legend,
      nodes near coords,
      legend style={legend pos=north east,font=\small, draw=none, legend columns=-1}
      ]

      \pgfplotstableread{data/ver-assert-iter-compariosn.dat}\unsoundness

      \addplot+[ybar, Blue, pattern color=Blue, pattern=north east lines]
          table[x expr=\coordindex, y=x5] from \unsoundness;

      \addplot+[ybar, Red, pattern color=Red, pattern=north west lines]
          table[x expr=\coordindex, y=x4] from \unsoundness;

      \legend{40 iterations, 80 iterations}
    \end{axis}
  \end{tikzpicture}
}
\vspace{-0.5em}
\caption{Comparison of the number of assertions verified with
  the best recipe generated by the different optimization algorithms,
  for different numbers of iterations.}
\label{fig:alg-iter-comparison}
\vspace{-0.5em}
\end{figure}


% -------------------- 40 80 avg iteration graph (5 min)
\begin{figure}[t]
\centering
\scalebox{0.75}{
  \begin{tikzpicture}
    \begin{axis}[
      % ybar stacked,
      ybar,
      xticklabels={\textsc{dars},\textsc{rs},\textsc{hc},\textsc{sa}},
      xtick=data,
      % xticklabel style={rotate=-45},
      ylabel={\textbf{Average number of iterations}},
      legend cell align=left,
      axis y line*=none,
      axis x line*=bottom,
      width=10cm,
      height=5.5cm,
      ymin=0,
      ymax=60,
      ytick distance=30,
      bar width=0.6cm,
      area legend,
      nodes near coords,
      legend style={legend pos=north east,font=\small, draw=none, legend columns=-1}
      % every node near coord/.append style={rotate=90, anchor=west}
      ]

      \pgfplotstableread{data/ver-assert-iter-4080compariosn.dat}\unsoundness

      \addplot+[ybar, Blue, pattern color=Blue, pattern=north east lines]
          table[x expr=\coordindex, y=x5] from \unsoundness;

      \addplot+[ybar, Red, pattern color=Red, pattern=north west lines]
          table[x expr=\coordindex, y=x4] from \unsoundness;

      \legend{40 iterations, 80 iterations}
    \end{axis}
  \end{tikzpicture}
}
\vspace{-0.5em}
\caption{Comparison of the average number of iterations that each
  algorithm needs to find the best recipe, for varying numbers of
  iterations.}
\label{fig:alg-iter-best-iterations}
\vspace{-1.0em}
\end{figure}

%% In comparison to RQ3, we now observed two additional combinations
%% of domains that are not natively supported in \crab. The
%% \texttt{zones} domain was combined with \texttt{term(int)} (4
%% occurrences). This is an interesting variant of the already
%% built-in combination of \texttt{zones} with \texttt{term(disInt)},
%% which is more precise.  We also found three combinations of a
%% convex and a non-convex domain, namely \texttt{polyhedra} with
%% \texttt{boxes} (5 occurrences), \texttt{octagons} with
%% \texttt{boxes} (6 occurrences) and \texttt{ric} with \texttt{boxes}
%% (1 occurrence).


The results show that, for our benchmarks, mutating the recipe found
by \textsc{dars} rarely led to an improvement. In particular, at least
93\% of all mutated recipes were either equal to or worse than the
original recipe. In the majority of these cases, mutated recipes are
equally good. This indicates that there are many optimal or
close-to-optimal solutions and that \textsc{dars} is able to find one
of them. This also explains why \textsc{rs} is very competitive.

\textbf{RQ7: Quantifying recipe optimality on different code
  versions.}
%
Computing an optimized recipe for every program version is
inefficient. We now show that a recipe optimized for one program
version is likely to also be optimal for another, even when the two
versions are 50 commits apart. This allows users of the abstract
interpreter or a CI system to re-apply optimized configurations.

To measure the optimality of a recipe across code versions, we took a
random sample of 60 files from our benchmark suite and retrieved the
50 most recent commits per file. We instrumented each file version
with the four assertion types described in \secref{subsec:Benchmarks}.
It should be noted that for some files we retrieved fewer than 50
versions, either because there were fewer than 50 total commits or our
build procedure for the project failed on earlier commits.

We analyzed each file version with the best recipe, $R_o$, found by
\textsc{dars} for the oldest file version. We compared this
recipe with new best recipes, $R_s$, that were generated by
\textsc{dars} when run on each subsequent file version. For this
experiment, we used the same setup as in RQ1. We selected the
\textsc{dars} optimization algorithm because it proved the most
assertions (\figref{fig:alg-comparison}).

Note that, when running \textsc{dars} with the same random seed, it
explores the same 40 recipes. It is, therefore, very likely that
if recipe $R_o$ for the oldest commit is the best (out of 40) for
one of the file versions, it is likely the best for
other file versions as well. To avoid any such bias, we performed this
experiment by seeding each run of \textsc{dars} with a different
random seed for each commit.
%
The results are shown in \figsref{fig:commits-different-seeds} and
\ref{fig:commits-loc-different-seeds}.

In \figref{fig:commits-different-seeds}, we give a bar chart comparing
the number of files per commit that have a positive, equal, and
negative difference in the number of verified assertions. An equal
difference means that the recipe for the oldest commit, $R_o$, proves
the same number of assertions in the current file version, $f_s$, as
the best recipe $R_s$ found by running \textsc{dars} on $f_s$. To be
more precise, we consider the two recipes to be equal if they differ
by at most 1 verified assertion or 1\% of verified assertions since
such a small change in the number of safe assertions seems acceptable
in practice (especially given that the total number of assertions may
change across commits). A positive difference in the figure means that
$R_o$ achieves better verification results than $R_s$, that is, $R_o$
proves more assertions safe (over 1 assertion or 1\% of the assertions
that $R_s$ proves). Analogously, a worse difference means that $R_o$
proves fewer assertions.
%
We do not consider time here because none of the recipes timed out
when applied on any file version.

Note that the number of files tends to decrease as the commit number
increases. This is because not all files go forward by 50 commits, and
even if they do, not all file versions build. However, in a few
instances, the number of files increases going forward in time. This
happens for files that change names, and later, change back, which we
do not catch.

% -------------------- Toggling best recipes
\begin{figure}[t]
\centering
\scalebox{0.75}{
\begin{tikzpicture}
\begin{axis}[
   ybar stacked,
     symbolic x coords={1, 2, 3, 4, 5, 6, 7},
	 xtick=data,
	 xticklabels={\textsc{dw}, \textsc{ni}, \textsc{wt}, \textsc{as}, \textsc{b}, \textsc{d}, \textsc{o}},
     ylabel={\textbf{Percentage of mutated recipes}},
     legend cell align=left,
     axis y line*=none,
     axis x line*=bottom,
     width=10cm,
     height=5.5cm,
     ymin=0,
     ymax=125,
     ytick distance=50,
     bar width=0.65cm,
     area legend,
     legend style={legend pos=north east,font=\small, draw=none, legend columns=-1}
   ]

\addplot+[ybar, DarkOrange!70] plot coordinates {(1,81.2) (2,90) (3,89.5) (4,69.9) (5,37.9) (6,14.2) (7,95.7)};

\addplot+[ybar, Red!70] plot coordinates {(1,10) (2,0.8) (3,1.4) (4,16.7) (5,57.1) (6,84) (7,4.3)};

\addplot+[ybar, Green!70] plot coordinates {(1,8.7) (2,8.8) (3,8.9) (4,13.3) (5,4.9) (6,1.7) (7, 0)};

\legend{Equal, Negative, Positive}
\end{axis}
\end{tikzpicture}
}
\vspace{-0.5em}
\caption{Effect of different settings on the precision and performance
  of the abstract interpreter. (\textsc{dw}: \delays, \textsc{ni}:
  \narrowings, \textsc{wt}: \thresholds, \textsc{as}: array smashing,
  \textsc{b}: backward analysis, \textsc{d}: abstract domain,
  \textsc{o}: ingredient ordering)}
\label{fig:toggle-best-recipe}
\vspace{-1em}
\end{figure}

As shown in the figure, for the vast majority of files, using recipe
$R_o$ (found for the oldest commit) is as effective as using $R_s$
(found for the current commit). The difference in safe assertions is
negative for less than a quarter of the files tested, with the average
negative difference among these files being around 22\% (i.e., $R_o$
proved 22\% fewer assertions than $R_s$ in these files). On the
remaining three quarters of the files tested however, $R_o$ proves at
least as many assertions as $R_s$, and thus, $R_o$ tends to be optimal
across code versions.

\figref{fig:commits-loc-different-seeds} shows the average difference
in the number of verified assertions per change in lines of code from
the oldest commit. Note that a positive (resp. negative) difference
represents that $R_o$ (resp. $R_s$) proves more assertions. The plot
clearly shows that for most files, regardless of lines changed, $R_o$
and $R_s$ are equally effective. Regarding the outliers shown in the
figure, we noticed that all commits with a difference of 50 safe
assertions or more modify one particular file from the \textsc{git}
project. In this case, $R_o$ is not as effective because the widening
and narrowing settings have very low values.

%% % ---------------------- Bar chart for the commit experiment with different seed (backward)
%% \begin{figure}[t]
%% \centering
%% \scalebox{0.75}{
%% \begin{tikzpicture}
%% \begin{axis}[
%%    ybar stacked,
%%      symbolic x coords={1, 2, 3, 4, 5, 6, 7, 8, 9, 10, 11, 12,
%%      					13, 14, 15, 16, 17, 18, 19, 20,
%%                       21, 22, 23, 24, 25, 26, 27, 28, 29, 30,
%%                       31, 32, 33, 34, 35, 36, 37, 38, 39, 40, 41,
%%                      42, 43, 44, 45, 46, 47, 48, 49, 50},
%% 	 xtick=data,
%% 	 xticklabels={1,,,,,,,,,10,,,,,,,,,,20,,,,,,,,,,30,,,,,,,,,,40,,,,,,,,,,50},
%%      ylabel={\textbf{Number of files}},
%%      xlabel={\textbf{Commit number}},
%%      legend cell align=left,
%%      axis y line*=none,
%%      axis x line*=bottom,
%%      width=10cm,
%%      height=5.5cm,
%%      ymin=0,
%%      ymax=60,
%%      ytick distance=10,
%%      bar width=0.08cm,
%%      area legend,
%%      legend style={legend pos=north east,font=\small, draw=none, legend columns=-1}
%%    ]

%%   \addplot+[ybar, Orange!80] plot coordinates {
%%     (1, 60) (2, 28) (3, 26) (4, 25) (5, 29) (6, 24) (7, 20) (8, 26) (9, 21) (10, 19) (11, 19) (12, 17) (13, 14) (14, 15) (15, 13) (16, 13) (17, 11) (18, 13) (19, 13) (20, 13) (21, 13) (22, 13) (23, 12) (24, 12) (25, 11) (26, 12) (27, 11) (28, 10) (29, 10) (30, 11) (31, 12) (32, 10) (33, 11) (34, 8) (35, 10) (36, 10) (37, 10) (38, 10) (39, 10) (40, 10) (41, 10) (42, 9) (43, 9) (44, 7) (45, 7) (46, 8) (47, 8) (48, 7) (49, 7) (50, 7)
%%   };
%%     %% (1,60) (2,36) (3,37) (4,35)
%%     %%     	(5,34) (6,34) (7,31) (8,29) (9,26) (10,24) (11,22)
%%     %%     	(12,23) (13,20) (14,20) (15,20) (16,19) (17,17) (18,16)
%%     %%     	(19,16) (20,15) (21,17) (22,16) (23,16)
%%     %%     	(24,15) (25,14) (26,15) (27,13) (28,13) (29,13) (30,13)
%%     %%     	(31,14) (32,13) (33,13) (34,12) (35,13) (36,12)
%%     %%     	(37,12) (38,11) (39,11) (40,10) (41,9) (42,9) (43,9)
%%     %%     	(44,8) (45,7) (46,8)
%%     %%     	(47,7) (48,8) (49,7) (50,8)};
%%   \addplot+[ybar, Red!70] plot coordinates {
%%     (1, 0) (2, 2) (3, 3) (4, 2) (5, 2) (6, 3) (7, 5) (8, 3) (9, 3) (10, 5) (11, 4) (12, 3) (13, 4) (14, 5) (15, 4) (16, 3) (17, 3) (18, 2) (19, 3) (20, 3) (21, 3) (22, 3) (23, 3) (24, 3) (25, 3) (26, 2) (27, 2) (28, 2) (29, 2) (30, 1) (31, 1) (32, 1) (33, 1) (34, 2) (35, 0) (36, 3) (37, 0) (38, 1) (39, 0) (40, 0) (41, 0) (42, 0) (43, 1) (44, 0) (45, 2) (46, 1) (47, 0) (48, 0) (49, 0) (50, 1)
%%   };
%%     %% (1,0) (2,1) (3,2) (4,1)
%%     %%     	(5,0) (6,0) (7,2) (8,2) (9,2) (10,3)
%%     %%     	(11,4) (12,1) (13,2) (14,2) (15,2) (16,2) (17,2)
%%     %%     	(18,2) (19,2) (20,2) (21,2) (22,2) (23,2)
%%     %%     	(24,2) (25,2) (26,1) (27,1) (28,1) (29,1) (30,1)
%%     %%     	(31,0) (32,1) (33,1) (34,1) (35,0) (36,1)
%%     %%     	(37,0) (38,0) (39,0) (40,0) (41,0) (42,0) (43,0)
%%     %%     	(44,0) (45,1) (46,0)
%%     %%     	(47,0) (48,0) (49,0) (50,0)};
%%   \addplot+[ybar, Green!70] plot coordinates {
%%     (1, 0) (2, 11) (3, 11) (4, 11) (5, 6) (6, 9) (7, 9) (8, 4) (9, 6) (10, 4) (11, 3) (12, 4) (13, 4) (14, 2) (15, 5) (16, 6) (17, 5) (18, 4) (19, 2) (20, 2) (21, 3) (22, 2) (23, 3) (24, 2) (25, 2) (26, 2) (27, 1) (28, 2) (29, 2) (30, 2) (31, 1) (32, 3) (33, 2) (34, 3) (35, 3) (36, 0) (37, 2) (38, 0) (39, 1) (40, 1) (41, 0) (42, 1) (43, 0) (44, 2) (45, 0) (46, 0) (47, 0) (48, 1) (49, 0) (50, 0)
%%   };
%% %%       (1,0) (2,3) (3,0)
%% %% (4,1) (5,2) (6,2) (7,1) (8,2) (9,2) (10,1)
%% %% 		(11,0) (12,0) (13,0) (14,0) (15,0) (16,1) (17,0)
%% %% 		(18,1) (19,0) (20,1) (21,0) (22,0) (23,0)
%% %% 		(24,0) (25,0) (26,0) (27,0) (28,0) (29,0) (30,0)
%% %% 		(31,0) (32,0) (33,0) (34,1) (35,1) (36,1)
%% %% 		(37,1) (38,1) (39,1) (40,1) (41,1) (42,1) (43,1)
%% %% 		(44,1) (45,1) (46,1)
%% %% 		(47,1) (48,0) (49,0) (50,0)};
%% \legend{Equal, Negative, Positive}
%% \end{axis}
%% \end{tikzpicture}
%% }
%% \vspace{-1em}
%% \caption{Difference in the ratio of safe vs. total assertions across
%%    commits.}
%% \label{fig:commits-different-seeds}
%% \vspace{-0.5em}
%% \end{figure}

% ---------------------- Bar chart for the commit experiment with different seed (forward)
\begin{figure}[t]
\centering
\scalebox{0.75}{
\begin{tikzpicture}
\begin{axis}[
   ybar stacked,
     %% symbolic x coords={1, 2, 3, 4, 5, 6, 7, 8, 9, 10, 11, 12,
     %% 					13, 14, 15, 16, 17, 18, 19, 20,
     %%                  21, 22, 23, 24, 25, 26, 27, 28, 29, 30,
     %%                  31, 32, 33, 34, 35, 36, 37, 38, 39, 40, 41,
     %%                 42, 43, 44, 45, 46, 47, 48, 49, 50},
   symbolic x coords={0, 1, 2, 3, 4, 5, 6, 7, 8, 9, 10, 11, 12,
     					13, 14, 15, 16, 17, 18, 19, 20,
                      21, 22, 23, 24, 25, 26, 27, 28, 29, 30,
                      31, 32, 33, 34, 35, 36, 37, 38, 39, 40, 41,
                     42, 43, 44, 45, 46, 47, 48, 49},
	 xtick=data,
	 %% xticklabels={1,,,,,,,,,10,,,,,,,,,,20,,,,,,,,,,30,,,,,,,,,,40,,,,,,,,,,50},
	 xticklabels={0,,,,,,,,,9,,,,,,,,,,19,,,,,,,,,,29,,,,,,,,,,39,,,,,,,,,,49},
     ylabel={\textbf{Number of files}},
     xlabel={\textbf{Commits after oldest commit}},
     legend cell align=left,
     axis y line*=none,
     axis x line*=bottom,
     width=10cm,
     height=5.5cm,
     ymin=0,
     ymax=60,
     ytick distance=10,
     bar width=0.08cm,
     area legend,
     legend style={legend pos=north east,font=\small, draw=none, legend columns=-1}
   ]

  \addplot+[ybar, Orange!80] plot coordinates {
    % # Safe <= 1% or # Safe <= 1 (absolute and relative)
    (0, 60) (1, 39) (2, 38) (3, 35) (4, 29) (5, 26) (6, 24) (7, 25) (8, 24) (9, 24) (10, 22) (11, 21) (12, 17) (13, 17) (14, 16) (15, 18) (16, 14) (17, 15) (18, 15) (19, 16) (20, 16) (21, 13) (22, 12) (23, 12) (24, 11) (25, 11) (26, 9) (27, 9) (28, 9) (29, 8) (30, 8) (31, 9) (32, 10) (33, 9) (34, 9) (35, 9) (36, 9) (37, 8) (38, 8) (39, 8) (40, 6) (41, 8) (42, 7) (43, 7) (44, 7) (45, 7) (46, 6) (47, 6) (48, 5) (49, 6)
    %% # Safe <= 1% (relative)
    %% (0, 60) (1, 32) (2, 32) (3, 31) (4, 26) (5, 22) (6, 17) (7, 21) (8, 19) (9, 18) (10, 19) (11, 19) (12, 15) (13, 14) (14, 13) (15, 14) (16, 11) (17, 12) (18, 12) (19, 13) (20, 13) (21, 12) (22, 11) (23, 10) (24, 11) (25, 10) (26, 8) (27, 8) (28, 8) (29, 7) (30, 8) (31, 8) (32, 7) (33, 7) (34, 8) (35, 8) (36, 7) (37, 7) (38, 8) (39, 8) (40, 6) (41, 8) (42, 7) (43, 5) (44, 6) (45, 6) (46, 6) (47, 5) (48, 5) (49, 6)
    % # Safe <= 1 (absolute)
    %% (0, 60) (1, 39) (2, 38) (3, 35) (4, 29) (5, 25) (6, 23) (7, 24) (8, 23) (9, 23) (10, 22) (11, 21) (12, 17) (13, 17) (14, 16) (15, 17) (16, 14) (17, 14) (18, 15) (19, 15) (20, 15) (21, 12) (22, 11) (23, 11) (24, 10) (25, 10) (26, 8) (27, 8) (28, 8) (29, 7) (30, 7) (31, 8) (32, 9) (33, 8) (34, 8) (35, 8) (36, 9) (37, 7) (38, 8) (39, 7) (40, 6) (41, 8) (42, 7) (43, 7) (44, 7) (45, 7) (46, 6) (47, 6) (48, 5) (49, 6)
    % Safe ratio diff <= 0.05 (original)
    %% (0, 60) (1, 39) (2, 39) (3, 37) (4, 30) (5, 29) (6, 26) (7, 26) (8, 25) (9, 26) (10, 23) (11, 21) (12, 18) (13, 19) (14, 17) (15, 17) (16, 14) (17, 14) (18, 15) (19, 15) (20, 15) (21, 13) (22, 12) (23, 12) (24, 12) (25, 12) (26, 9) (27, 10) (28, 10) (29, 9) (30, 10) (31, 10) (32, 10) (33, 9) (34, 8) (35, 8) (36, 9) (37, 7) (38, 8) (39, 7) (40, 6) (41, 8) (42, 7) (43, 7) (44, 7) (45, 7) (46, 6) (47, 6) (48, 5) (49, 6)
  };
  \addplot+[ybar, Red!70] plot coordinates {
    % # Safe <= 1% or # Safe <= 1 (absolute and relative)
    (0, 0) (1, 2) (2, 3) (3, 4) (4, 8) (5, 7) (6, 7) (7, 8) (8, 4) (9, 6) (10, 4) (11, 2) (12, 4) (13, 4) (14, 5) (15, 4) (16, 4) (17, 3) (18, 4) (19, 3) (20, 3) (21, 5) (22, 5) (23, 5) (24, 5) (25, 5) (26, 5) (27, 5) (28, 5) (29, 5) (30, 5) (31, 5) (32, 4) (33, 5) (34, 5) (35, 5) (36, 4) (37, 4) (38, 4) (39, 3) (40, 4) (41, 2) (42, 3) (43, 2) (44, 2) (45, 2) (46, 2) (47, 2) (48, 3) (49, 2)
    % # Safe <= 1% (relative)
    %% (0, 0) (1, 3) (2, 5) (3, 6) (4, 8) (5, 8) (6, 8) (7, 10) (8, 6) (9, 9) (10, 6) (11, 3) (12, 5) (13, 6) (14, 7) (15, 6) (16, 5) (17, 4) (18, 5) (19, 4) (20, 5) (21, 5) (22, 5) (23, 5) (24, 5) (25, 5) (26, 5) (27, 5) (28, 5) (29, 5) (30, 5) (31, 5) (32, 5) (33, 5) (34, 5) (35, 5) (36, 4) (37, 5) (38, 4) (39, 3) (40, 4) (41, 2) (42, 3) (43, 3) (44, 3) (45, 3) (46, 2) (47, 2) (48, 3) (49, 2)
    % # Safe <= 1 (absolute)
    %% (0, 0) (1, 2) (2, 3) (3, 4) (4, 8) (5, 8) (6, 8) (7, 9) (8, 5) (9, 7) (10, 4) (11, 2) (12, 4) (13, 4) (14, 5) (15, 5) (16, 4) (17, 4) (18, 4) (19, 4) (20, 4) (21, 6) (22, 6) (23, 6) (24, 6) (25, 6) (26, 6) (27, 6) (28, 6) (29, 6) (30, 6) (31, 6) (32, 5) (33, 6) (34, 6) (35, 6) (36, 4) (37, 5) (38, 4) (39, 4) (40, 4) (41, 2) (42, 3) (43, 2) (44, 2) (45, 2) (46, 2) (47, 2) (48, 3) (49, 2)
    % Safe ratio diff <= 0.05 (original)
    %% (0, 0) (1, 2) (2, 2) (3, 3) (4, 7) (5, 5) (6, 6) (7, 7) (8, 3) (9, 4) (10, 3) (11, 2) (12, 3) (13, 2) (14, 4) (15, 5) (16, 4) (17, 4) (18, 4) (19, 4) (20, 4) (21, 5) (22, 5) (23, 5) (24, 4) (25, 4) (26, 5) (27, 4) (28, 4) (29, 5) (30, 4) (31, 4) (32, 4) (33, 5) (34, 6) (35, 6) (36, 4) (37, 5) (38, 4) (39, 4) (40, 4) (41, 2) (42, 3) (43, 2) (44, 2) (45, 2) (46, 2) (47, 2) (48, 3) (49, 2)
  };
  \addplot+[ybar, Green!70] plot coordinates {
    % # Safe <= 1% or # Safe <= 1 (absolute and relative)
    (0, 0) (1, 2) (2, 1) (3, 2) (4, 0) (5, 1) (6, 1) (7, 0) (8, 0) (9, 0) (10, 0) (11, 0) (12, 0) (13, 0) (14, 0) (15, 0) (16, 0) (17, 0) (18, 0) (19, 0) (20, 0) (21, 0) (22, 1) (23, 0) (24, 0) (25, 0) (26, 0) (27, 0) (28, 0) (29, 1) (30, 1) (31, 0) (32, 0) (33, 0) (34, 0) (35, 0) (36, 0) (37, 0) (38, 0) (39, 0) (40, 0) (41, 0) (42, 0) (43, 0) (44, 0) (45, 0) (46, 0) (47, 0) (48, 0) (49, 0)
    % # Safe <= 1% (relative)
    %% (0, 0) (1, 8) (2, 5) (3, 4) (4, 3) (5, 4) (6, 7) (7, 2) (8, 3) (9, 3) (10, 1) (11, 1) (12, 1) (13, 1) (14, 1) (15, 2) (16, 2) (17, 2) (18, 2) (19, 2) (20, 1) (21, 1) (22, 2) (23, 2) (24, 0) (25, 1) (26, 1) (27, 1) (28, 1) (29, 2) (30, 1) (31, 1) (32, 2) (33, 2) (34, 1) (35, 1) (36, 2) (37, 0) (38, 0) (39, 0) (40, 0) (41, 0) (42, 0) (43, 1) (44, 0) (45, 0) (46, 0) (47, 1) (48, 0) (49, 0)
    % # Safe <= 1 (absolute)
    %% (0, 0) (1, 2) (2, 1) (3, 2) (4, 0) (5, 1) (6, 1) (7, 0) (8, 0) (9, 0) (10, 0) (11, 0) (12, 0) (13, 0) (14, 0) (15, 0) (16, 0) (17, 0) (18, 0) (19, 0) (20, 0) (21, 0) (22, 1) (23, 0) (24, 0) (25, 0) (26, 0) (27, 0) (28, 0) (29, 1) (30, 1) (31, 0) (32, 0) (33, 0) (34, 0) (35, 0) (36, 0) (37, 0) (38, 0) (39, 0) (40, 0) (41, 0) (42, 0) (43, 0) (44, 0) (45, 0) (46, 0) (47, 0) (48, 0) (49, 0)
    % Safe ratio diff <= 0.05 (original)   
    %% (0, 0) (1, 2) (2, 1) (3, 1) (4, 0) (5, 0) (6, 0) (7, 0) (8, 0) (9, 0) (10, 0) (11, 0) (12, 0) (13, 0) (14, 0) (15, 0) (16, 0) (17, 0) (18, 0) (19, 0) (20, 0) (21, 0) (22, 1) (23, 0) (24, 0) (25, 0) (26, 0) (27, 0) (28, 0) (29, 0) (30, 0) (31, 0) (32, 0) (33, 0) (34, 0) (35, 0) (36, 0) (37, 0) (38, 0) (39, 0) (40, 0) (41, 0) (42, 0) (43, 0) (44, 0) (45, 0) (46, 0) (47, 0) (48, 0) (49, 0)
  };
\legend{Equal, Negative, Positive}
\end{axis}
\end{tikzpicture}
}
\vspace{-1em}
\caption{Difference in the safe assertions across commits.}
\label{fig:commits-different-seeds}
\vspace{-0.5em}
\end{figure}


% -------- Scatter plot for the commit experiment with different seed
\begin{figure}[t]
\centering
\scalebox{0.75}{
\begin{tikzpicture}
  \pgfplotsset{
      scale only axis,
  }

  \begin{axis}[
      xlabel=\vspace{0.5em}\textbf{LOC difference from oldest commit},
   % AVERAGE PERCENTAGE DIFFERENCE      
      %% ylabel style={align=center}, ylabel=\textbf{Average percentage difference}\\\textbf{from oldest difference},
   % AVERAGE ABSOLUTE DIFFERENCE      
      ylabel style={align=center}, ylabel=\textbf{Average difference in safe assertions}\\\textbf{from oldest commit},
   % AVERAGE RELATIVE DIFFERENCE      
      %% ylabel style={align=center}, ylabel=\textbf{Average difference in ratio of}\\\textbf{safe assertions from oldest commit},
  ]


   % AVERAGE PERCENTAGE DIFFERENCE
    %% \pgfplotstableread[col sep = comma]{data/loc-diff-forward-orig.csv}\scatterplot
   % AVERAGE ABSOLUTE DIFFERENCE
    \pgfplotstableread[col sep = comma]{data/loc-diff-forward-abs.csv}\scatterplot
   % AVERAGE RELATIVE DIFFERENCE
    %% \pgfplotstableread[col sep = comma]{data/loc-diff-forward-rel.csv}\scatterplot
  \addplot[scatter, only marks] table [x=xax, y=yax, col sep=comma] {\scatterplot};



  \end{axis}
\end{tikzpicture}
}
\vspace{-0.5em}
\caption{Average difference in the number of safe assertions per
  change in lines of code from the oldest commit.}
\label{fig:commits-loc-different-seeds}
\vspace{-0.5em}
\end{figure}


%% ----------------------------------------------------------------
\subsection{Threats to Validity}
\label{subsec:Threats}
%% ----------------------------------------------------------------

We have identified the following threats to the validity of our
experiments.

\textbf{Benchmark selection.} Our results may not generalize to other
benchmarks. However, we selected popular GitHub projects from
different application domains (see \tabref{tab:projects}).
%
Hence, we believe that our benchmark selection mitigates this threat
and increases generalizability of our findings.

\textbf{Abstract interpreter and recipe settings.} For our
experiments, we only used a single abstract interpreter, \crab, which
however is a mature tool and actively supported.
%
The selection of recipe settings was, of course, influenced by the
available settings in \crab. Nevertheless, \crab implements the
generic architecture of \figref{fig:interpreter}, used by most
abstract interpreters, such as those mentioned at the beginning of
\secref{sec:abstract-interpreters}. We, therefore, expect our approach
to generalize to such analyzers.

\textbf{Optimization algorithms.} We considered four optimization
algorithms, but in \secref{sec:Algorithms}, we explain why these are
suitable for our application domain.

\textbf{Assertion types.} Our results are based on four types of assertions. However, they
cover a broad spectrum of runtime errors that are commonly checked by static analyzers.

